NWChem: Past, Present, and Future

Specialized computational chemistry packages have permanently reshaped the landscape of chemical and materials science by providing tools to support and guide experimental efforts and for the prediction of atomistic and electronic properties. In this regard, electronic structure packages have played a special role by using first-principledriven methodologies to model complex chemical and materials processes. Over the last few decades, the rapid development of computing technologies and the tremendous increase in computational power have offered a unique chance to study complex transformations using sophisticated and predictive many-body techniques that describe correlated behavior of electrons in molecular and condensed phase systems at different levels of theory. In enabling these simulations, novel parallel algorithms have been able to take advantage of computational resources to address the polynomial scaling of electronic structure methods. In this paper, we briefly review the NWChem computational chemistry suite, including its history, design principles, parallel tools, current capabilities, outreach and outlook.

==> ccsdt-performance.tex <==
The parallel implementation of the CCSD(T) approach by  Kobayashi and Rendell \cite{Kobayashi}, employing the spin adaptation scheme based on the unitary group approach (UGA) 
\cite{Scuseria} within NWChem, was one of the  first scalable  implementations of the 
CC formalism  capable of taking advantage of several hundred processors.
This implementation was  used in 
simulations involving tera- and peta-scale architectures where chemical accuracy is required to
describe ground-state potential energy surfaces. One of the best illustrations of the performance of the CCSD(T) implementation is provided by
 calculations for water clusters \cite{apra2009liquid}. In  the largest calculation,  (H$_2$O)$_{24}$, sustained performance of 1.39 
PetaFLOP/s (double precision) on 223,200 processors of ORNL's Jaguar system  was documented. 
This impressive performance was mostly 
attributed to the (T)-part characterized by $n_o^3n_u^4$ numerical overhead (where $n_o$ and $n_u$ refer to the total numbers of correlated occupied and virtual orbitals)  and its relatively low communication footprint. \\
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.47]{closed_shell_cc.pdf}
%\caption{Wall-time of the CCSD(T) calculations of total energy of (H$_2$O)$_{24}$ as a function of the processor number.}
%\label{closedcc}
%\end{figure}


==> cmd-rlins.tex <==
Integration of classical and quantum mechanical tools in NWChem allows one to develop accurate force field parameters (point charges,
bonded potentials and van der Waals coefficients) to be used in
classical molecular dynamics simulations. Over the last 20 years,
classical parameters obtained using NWChem have been employed to
address the underlying mechanisms of a variety of novel complex
biological systems and their interactions (e.g., lipopolysaccharide
membranes, carbohydrate moieties, mineral surfaces, radionuclides,
organophosphorous compounds)\cite{Lins2001,Lins2008,Soares2008b,
doi:10.1021/ct700024h,Shroll2002,Shroll2003a,doi:10.1021/jp208787g,
doi:10.1021/jp9083635,doi:10.1021/es702688c,doi:10.1021/jp906124a}
 which led to a significant expansion
of the database of AMBER- and Glycam-compatible force fields. In
addition, it has also shaped the newer generation of lipids,
carbohydrates and nucleic acids of the officially distributed GROMOS
force field\cite{Chandrasekhar2003,doi:10.1002/jcc.20275,doi:10.1021/ct300479h,
doi:10.1002/jcc.23721,doi:10.1002/jcc.20193,doi:10.1002/bip.21602,
doi:10.1021/ct8002964}

